A Review and Comparative Study on Probabilistic Object Detection in Autonomous Driving

Capturing uncertainty in object detection is indispensable for safe autonomous driving. In recent years, deep learning has become the de-facto approach for object detection, and many probabilistic object detectors have been proposed. However, there is no summary on uncertainty estimation in deep object detection, and existing methods are not only built with different network architectures and uncertainty estimation methods, but also evaluated on different datasets with a wide range of evaluation metrics. As a result, a comparison among methods remains challenging, as does the selection of a model that best suits a particular application. This paper aims to alleviate this problem by providing a review and comparative study on existing probabilistic object detection methods for autonomous driving applications. First, we provide an overview of generic uncertainty estimation in deep learning, and then systematically survey existing methods and evaluation metrics for probabilistic object detection. Next, we present a strict comparative study for probabilistic object detection based on an image detector and three public autonomous driving datasets. Finally, we present a discussion of the remaining challenges and future works. Code has been made available at https://github.com/asharakeh/pod_compare.git

==> Object_detection_table.tex <==
\captionsetup{font=normalsize}
\scriptsize
\centering
\begin{threeparttable}
\begin{tabularx}{1.00\linewidth}{
>{\raggedright\arraybackslash\hsize=0.2\hsize}X % reference
>{\raggedright\arraybackslash\hsize=0.1\hsize}X % year
>{\raggedright\arraybackslash\hsize=0.1\hsize}X % sensors
>{\raggedright\arraybackslash\hsize=0.3\hsize}X % obj. type
>{\raggedright\arraybackslash\hsize=0.3\hsize}X % dataset
>{\raggedright\arraybackslash\hsize=0.15\hsize}X % unc.type
>{\raggedright\arraybackslash\hsize=0.2\hsize}X % unc. method
>{\raggedright\arraybackslash\hsize=0.3\hsize}X % unc. cls.
>{\raggedright\arraybackslash\hsize=0.4\hsize}X % unc. reg.
>{\raggedright\arraybackslash\hsize=0.3\hsize}X % post-processing
} 
\caption{A summary of probabilistic object detection networks}\label{tab:summary_object_detection}\\
\rowcolor{lightgray!25}
\textbf{Reference} &  \textbf{Year} & \textbf{Sen.} & \textbf{Obj. Type} & \textbf{Dataset} & \textbf{Unc. Type} & \textbf{Unc. Method} & \textbf{Unc. Cls.} & \textbf{Unc. Reg.} & \textbf{Post-proc.} \\[4pt]
\endhead

% Towards Safe Autonomous Driving: Capture Uncertainty in the Deep Neural Network For Lidar 3D Vehicle Detection
Feng \etal~\cite{feng2018towards} & 2018 & L & 3D vehicles & KITTI & E+A & MC-dropout, Direct-Mod. & Sofmtax & Multivariate Gaussian with diagonal covariance matrix & Std. NMS \\
% Leveraging Heteroscedastic Aleatoric Uncertainties for Robust Real-Time LiDAR 3D Object Detection
Feng \etal~\cite{feng2018leveraging} & 2018 & L & 3D car & KITTI & A & Direct-Mod. & Softmax & Multivariate Gaussian with diagonal covariance matrix. & Std. NMS \\
% Deep Active Learning for Efficient Training of a LiDAR 3D Object Detector
Feng \etal~\cite{feng2019deep} & 2019 & L+C & 3D multi-class & KITTI & E & MC-dropout, Deep Ensembles & Softmax & - & Std. NMS \\
% Can We Trust You? On Calibration of a Probabilistic Object Detector for Autonomous Driving
Feng \etal~\cite{feng2019can} & 2019 & L & 3D car & KITTI, NuScenes & A & Direct-Mod. & Softmax & Multivariate Gaussian with diagonal covariance matrix. & Std. NMS \\
% Leveraging Uncertainties for Deep Multi-modal Object Detection in Autonomous Driving
Feng \etal~\cite{feng2020leveraging} & 2020 & L+C & 3D car & KITTI, NuScenes, Bosch & A & Direct-mod. & Softmax, univariate Gaussian & Multivariate Gaussian with diagonal covariance matrix & Std. NMS \\ 
% Uncertainty Estimation in One-Stage Object Detection
Kraus \etal~\cite{kraus2019uncertainty} & 2019 & C & 2D Pedestrians, Riders & EuroCity Persons & E+A & MC-dropout, Direct-mod. & Softmax & Multivariate Gaussian with diagonal covariance matrix. & Std. NMS\\ 
% Uncertainty estimation for deep neural object detectors in safety-critical applications
Le \etal~\cite{le2018uncertainty} & 2018 & C & 2D multi-class & KITTI & A & Direct-mod. & Softmax & Multivariate Gaussian with diagonal covariance matrix & Std. NMS, Anchor Statistics \\ 
% Dropout Sampling for Robust Object Detection in Open-Set Conditions
Miller \etal~\cite{miller2018dropout} & 2018 & C & 2D multi-class & COCO, SceneNet RGBD, QUT Campus Dataset & E & MC-dropout & Softmax & - & Std. NMS \\ 
% Evaluating merging strategies for sampling-based uncertainty techniques in object detection
Miller \etal~\cite{miller2019evaluating} & 2019 & C & 2D multi-class & COCO, PASCAL-VOC, Underwater Scenes & E & MC-dropout & Softmax & Multivariate Gaussian with diagonal covariance matrix & Std. NMS \\ 
% Bounding box regression with uncertainty for accurate object detection
He \etal~\cite{he2019bounding} & 2019 & C & 2D multi-class & COCO, PASCAL-VOC & A & Direct-Mod. & Softmax & Multivariate Gaussian with diagonal covariance matrix & Std. NMS \\
% BayesOD: A Bayesian Approach for Uncertainty Estimation in Deep Object Detectors
Harakeh \etal~\cite{harakeh2019bayesod} & 2020 & C & 2D multi-class & COCO, PASCAL-VOC, BDD, KITTI & E+A & MC-dropout, Direct-Mod. & Softmax & Multivariate Gaussian with diagonal covariance matrix & Bayesian Fusion \\
%Gaussian YOLOv3: An Accurate and Fast Object Detector Using Localization Uncertainty for Autonomous Driving
Choi \etal~\cite{choi2019gaussian} & 2019 & C & 2D multi-class & BDD, KITTI & A & Direct-Mod. & Softmax & Multivariate Gaussian with diagonal covariance matrix & Modified NMS \\
%Benchmarking Sampling-based Probabilistic Object Detectors
Miller \etal~\cite{miller2019benchmarking} & 2019 & C & 2D multi-class & COCO & E & MC-Dropout, Deep Ensembles & Softmax & - & Std. NMS\\
\bottomrule
\end{tabularx}

%\begin{tablenotes}
%\item[a] Some methods compare multiple fusion levels. We mark the fusion level with the best reported performance in bold.
%\item[b] They also test the methods for object detection problem with different network architectures (see Table~\ref{tab:object_detection_summary}). 
%\end{tablenotes}
\end{threeparttable}

